Two-Sample Testing for Event Impacts in Time Series

In many application domains, time series are monitored to detect extreme events like technical faults, natural disasters, or disease outbreaks. Unfortunately, it is often non-trivial to select both a time series that is informative about events and a powerful detection algorithm: detection may fail because the detection algorithm is not suitable, or because there is no shared information between the time series and the events of interest. In this work, we thus propose a non-parametric statistical test for shared information between a time series and a series of observed events. Our test allows identifying time series that carry information on event occurrences without committing to a specific event detection methodology. In a nutshell, we test for divergences of the value distributions of the time series at increasing lags after event occurrences with a multiple two-sample testing approach. In contrast to related tests, our approach is applicable for time series over arbitrary domains, including multivariate numeric, strings or graphs. We perform a large-scale simulation study to show that it outperforms or is on par with related tests on our task for univariate time series. We also demonstrate the real-world applicability of our approach on datasets from social media and smart home environments.

==> ms-gnuplottex-fig1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(9800.00,4320.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(94,3196){\makebox(0,0)[r]{\strut{}\scriptsize{-15}}}%
      \csname LTb\endcsname%%
      \put(94,3352){\makebox(0,0)[r]{\strut{}\scriptsize{-10}}}%
      \csname LTb\endcsname%%
      \put(94,3508){\makebox(0,0)[r]{\strut{}\scriptsize{-5}}}%
      \csname LTb\endcsname%%
      \put(94,3665){\makebox(0,0)[r]{\strut{}\scriptsize{0}}}%
      \csname LTb\endcsname%%
      \put(94,3821){\makebox(0,0)[r]{\strut{}\scriptsize{5}}}%
      \csname LTb\endcsname%%
      \put(94,3977){\makebox(0,0)[r]{\strut{}\scriptsize{10}}}%
      \csname LTb\endcsname%%
      \put(94,4133){\makebox(0,0)[r]{\strut{}\scriptsize{15}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(3233,3010){\makebox(0,0){\strut{}\scriptsize{time series with event impacts in mean}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(6758,3475){\makebox(0,0)[r]{\strut{}\scriptsize{-15}}}%
      \csname LTb\endcsname%%
      \put(6758,3585){\makebox(0,0)[r]{\strut{}\scriptsize{-10}}}%
      \csname LTb\endcsname%%
      \put(6758,3694){\makebox(0,0)[r]{\strut{}\scriptsize{-5}}}%
      \csname LTb\endcsname%%
      \put(6758,3804){\makebox(0,0)[r]{\strut{}\scriptsize{0}}}%
      \csname LTb\endcsname%%
      \put(6758,3914){\makebox(0,0)[r]{\strut{}\scriptsize{5}}}%
      \csname LTb\endcsname%%
      \put(6758,4023){\makebox(0,0)[r]{\strut{}\scriptsize{10}}}%
      \csname LTb\endcsname%%
      \put(6758,4133){\makebox(0,0)[r]{\strut{}\scriptsize{15}}}%
      \csname LTb\endcsname%%
      \put(7117,3289){\makebox(0,0){\strut{}\scriptsize{1}}}%
      \csname LTb\endcsname%%
      \put(7289,3289){\makebox(0,0){\strut{}\scriptsize{2}}}%
      \csname LTb\endcsname%%
      \put(7460,3289){\makebox(0,0){\strut{}\scriptsize{3}}}%
      \csname LTb\endcsname%%
      \put(7631,3289){\makebox(0,0){\strut{}\scriptsize{4}}}%
      \csname LTb\endcsname%%
      \put(7803,3289){\makebox(0,0){\strut{}\scriptsize{5}}}%
      \csname LTb\endcsname%%
      \put(7974,3289){\makebox(0,0){\strut{}\scriptsize{6}}}%
      \csname LTb\endcsname%%
      \put(8146,3289){\makebox(0,0){\strut{}\scriptsize{7}}}%
      \csname LTb\endcsname%%
      \put(8317,3289){\makebox(0,0){\strut{}\scriptsize{8}}}%
      \csname LTb\endcsname%%
      \put(8489,3289){\makebox(0,0){\strut{}\scriptsize{9}}}%
      \csname LTb\endcsname%%
      \put(8660,3289){\makebox(0,0){\strut{}\scriptsize{10}}}%
      \csname LTb\endcsname%%
      \put(8832,3289){\makebox(0,0){\strut{}\scriptsize{11}}}%
      \csname LTb\endcsname%%
      \put(9003,3289){\makebox(0,0){\strut{}\scriptsize{12}}}%
      \csname LTb\endcsname%%
      \put(9174,3289){\makebox(0,0){\strut{}\scriptsize{13}}}%
      \csname LTb\endcsname%%
      \put(9346,3289){\makebox(0,0){\strut{}\scriptsize{14}}}%
      \csname LTb\endcsname%%
      \put(9517,3289){\makebox(0,0){\strut{}\scriptsize{15}}}%
      \colorrgb{0.90,0.62,0.00}%%
      \put(6843,4221){\makebox(0,0)[l]{\strut{}\tiny{event}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8231,3010){\makebox(0,0){\strut{}\scriptsize{distributions $k=1,\dotsc,15$ steps after events}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(94,1756){\makebox(0,0)[r]{\strut{}\scriptsize{-15}}}%
      \csname LTb\endcsname%%
      \put(94,1912){\makebox(0,0)[r]{\strut{}\scriptsize{-10}}}%
      \csname LTb\endcsname%%
      \put(94,2068){\makebox(0,0)[r]{\strut{}\scriptsize{-5}}}%
      \csname LTb\endcsname%%
      \put(94,2225){\makebox(0,0)[r]{\strut{}\scriptsize{0}}}%
      \csname LTb\endcsname%%
      \put(94,2381){\makebox(0,0)[r]{\strut{}\scriptsize{5}}}%
      \csname LTb\endcsname%%
      \put(94,2537){\makebox(0,0)[r]{\strut{}\scriptsize{10}}}%
      \csname LTb\endcsname%%
      \put(94,2693){\makebox(0,0)[r]{\strut{}\scriptsize{15}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(3233,1570){\makebox(0,0){\strut{}\scriptsize{time series with event impacts in variance}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(6758,2035){\makebox(0,0)[r]{\strut{}\scriptsize{-15}}}%
      \csname LTb\endcsname%%
      \put(6758,2145){\makebox(0,0)[r]{\strut{}\scriptsize{-10}}}%
      \csname LTb\endcsname%%
      \put(6758,2254){\makebox(0,0)[r]{\strut{}\scriptsize{-5}}}%
      \csname LTb\endcsname%%
      \put(6758,2364){\makebox(0,0)[r]{\strut{}\scriptsize{0}}}%
      \csname LTb\endcsname%%
      \put(6758,2474){\makebox(0,0)[r]{\strut{}\scriptsize{5}}}%
      \csname LTb\endcsname%%
      \put(6758,2583){\makebox(0,0)[r]{\strut{}\scriptsize{10}}}%
      \csname LTb\endcsname%%
      \put(6758,2693){\makebox(0,0)[r]{\strut{}\scriptsize{15}}}%
      \csname LTb\endcsname%%
      \put(7117,1849){\makebox(0,0){\strut{}\scriptsize{1}}}%
      \csname LTb\endcsname%%
      \put(7289,1849){\makebox(0,0){\strut{}\scriptsize{2}}}%
      \csname LTb\endcsname%%
      \put(7460,1849){\makebox(0,0){\strut{}\scriptsize{3}}}%
      \csname LTb\endcsname%%
      \put(7631,1849){\makebox(0,0){\strut{}\scriptsize{4}}}%
      \csname LTb\endcsname%%
      \put(7803,1849){\makebox(0,0){\strut{}\scriptsize{5}}}%
      \csname LTb\endcsname%%
      \put(7974,1849){\makebox(0,0){\strut{}\scriptsize{6}}}%
      \csname LTb\endcsname%%
      \put(8146,1849){\makebox(0,0){\strut{}\scriptsize{7}}}%
      \csname LTb\endcsname%%
      \put(8317,1849){\makebox(0,0){\strut{}\scriptsize{8}}}%
      \csname LTb\endcsname%%
      \put(8489,1849){\makebox(0,0){\strut{}\scriptsize{9}}}%
      \csname LTb\endcsname%%
      \put(8660,1849){\makebox(0,0){\strut{}\scriptsize{10}}}%
      \csname LTb\endcsname%%
      \put(8832,1849){\makebox(0,0){\strut{}\scriptsize{11}}}%
      \csname LTb\endcsname%%
      \put(9003,1849){\makebox(0,0){\strut{}\scriptsize{12}}}%
      \csname LTb\endcsname%%
      \put(9174,1849){\makebox(0,0){\strut{}\scriptsize{13}}}%
      \csname LTb\endcsname%%
      \put(9346,1849){\makebox(0,0){\strut{}\scriptsize{14}}}%
      \csname LTb\endcsname%%
      \put(9517,1849){\makebox(0,0){\strut{}\scriptsize{15}}}%
      \colorrgb{0.90,0.62,0.00}%%
      \put(6843,2781){\makebox(0,0)[l]{\strut{}\tiny{event}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8231,1570){\makebox(0,0){\strut{}\scriptsize{distributions $k=1,\dotsc,15$ steps after events}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(94,316){\makebox(0,0)[r]{\strut{}\scriptsize{-15}}}%
      \csname LTb\endcsname%%
      \put(94,472){\makebox(0,0)[r]{\strut{}\scriptsize{-10}}}%
      \csname LTb\endcsname%%
      \put(94,629){\makebox(0,0)[r]{\strut{}\scriptsize{-5}}}%
      \csname LTb\endcsname%%
      \put(94,785){\makebox(0,0)[r]{\strut{}\scriptsize{0}}}%
      \csname LTb\endcsname%%
      \put(94,941){\makebox(0,0)[r]{\strut{}\scriptsize{5}}}%
      \csname LTb\endcsname%%
      \put(94,1098){\makebox(0,0)[r]{\strut{}\scriptsize{10}}}%
      \csname LTb\endcsname%%
      \put(94,1254){\makebox(0,0)[r]{\strut{}\scriptsize{15}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(3233,130){\makebox(0,0){\strut{}\scriptsize{time series with event impacts in tails}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(6758,595){\makebox(0,0)[r]{\strut{}\scriptsize{-15}}}%
      \csname LTb\endcsname%%
      \put(6758,705){\makebox(0,0)[r]{\strut{}\scriptsize{-10}}}%
      \csname LTb\endcsname%%
      \put(6758,815){\makebox(0,0)[r]{\strut{}\scriptsize{-5}}}%
      \csname LTb\endcsname%%
      \put(6758,925){\makebox(0,0)[r]{\strut{}\scriptsize{0}}}%
      \csname LTb\endcsname%%
      \put(6758,1034){\makebox(0,0)[r]{\strut{}\scriptsize{5}}}%
      \csname LTb\endcsname%%
      \put(6758,1144){\makebox(0,0)[r]{\strut{}\scriptsize{10}}}%
      \csname LTb\endcsname%%
      \put(6758,1254){\makebox(0,0)[r]{\strut{}\scriptsize{15}}}%
      \csname LTb\endcsname%%
      \put(7117,409){\makebox(0,0){\strut{}\scriptsize{1}}}%
      \csname LTb\endcsname%%
      \put(7289,409){\makebox(0,0){\strut{}\scriptsize{2}}}%
      \csname LTb\endcsname%%
      \put(7460,409){\makebox(0,0){\strut{}\scriptsize{3}}}%
      \csname LTb\endcsname%%
      \put(7631,409){\makebox(0,0){\strut{}\scriptsize{4}}}%
      \csname LTb\endcsname%%
      \put(7803,409){\makebox(0,0){\strut{}\scriptsize{5}}}%
      \csname LTb\endcsname%%
      \put(7974,409){\makebox(0,0){\strut{}\scriptsize{6}}}%
      \csname LTb\endcsname%%
      \put(8146,409){\makebox(0,0){\strut{}\scriptsize{7}}}%
      \csname LTb\endcsname%%
      \put(8317,409){\makebox(0,0){\strut{}\scriptsize{8}}}%
      \csname LTb\endcsname%%
      \put(8489,409){\makebox(0,0){\strut{}\scriptsize{9}}}%
      \csname LTb\endcsname%%
      \put(8660,409){\makebox(0,0){\strut{}\scriptsize{10}}}%
      \csname LTb\endcsname%%
      \put(8832,409){\makebox(0,0){\strut{}\scriptsize{11}}}%
      \csname LTb\endcsname%%
      \put(9003,409){\makebox(0,0){\strut{}\scriptsize{12}}}%
      \csname LTb\endcsname%%
      \put(9174,409){\makebox(0,0){\strut{}\scriptsize{13}}}%
      \csname LTb\endcsname%%
      \put(9346,409){\makebox(0,0){\strut{}\scriptsize{14}}}%
      \csname LTb\endcsname%%
      \put(9517,409){\makebox(0,0){\strut{}\scriptsize{15}}}%
      \colorrgb{0.90,0.62,0.00}%%
      \put(6843,1342){\makebox(0,0)[l]{\strut{}\tiny{event}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8231,130){\makebox(0,0){\strut{}\scriptsize{distributions $k=1,\dotsc,15$ steps after events}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{ms-gnuplottex-fig1}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> ms-gnuplottex-fig2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4800.00,11840.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(204,9475){\makebox(0,0)[r]{\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(204,9819){\makebox(0,0)[r]{\strut{}\tiny{0.2}}}%
      \csname LTb\endcsname%%
      \put(204,10163){\makebox(0,0)[r]{\strut{}\tiny{0.4}}}%
      \csname LTb\endcsname%%
      \put(204,10507){\makebox(0,0)[r]{\strut{}\tiny{0.6}}}%
      \csname LTb\endcsname%%
      \put(204,10851){\makebox(0,0)[r]{\strut{}\tiny{0.8}}}%
      \csname LTb\endcsname%%
      \put(204,11195){\makebox(0,0)[r]{\strut{}\tiny{1}}}%
      \csname LTb\endcsname%%
      \put(694,9289){\makebox(0,0){\strut{}\tiny{8}}}%
      \csname LTb\endcsname%%
      \put(1276,9289){\makebox(0,0){\strut{}\tiny{64}}}%
      \csname LTb\endcsname%%
      \put(1858,9289){\makebox(0,0){\strut{}\tiny{512}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1276,9010){\makebox(0,0){\strut{}\small{impact order $q$}}}%
      \csname LTb\endcsname%%
      \put(1276,11560){\makebox(0,0){\strut{}\small{Mean impact model}}}%
      \csname LTb\endcsname%%
      \put(788,9969){\makebox(0,0)[l]{\strut{}\tiny{GC-VAR}}}%
      \csname LTb\endcsname%%
      \put(788,9849){\makebox(0,0)[l]{\strut{}\tiny{TE-KSG}}}%
      \csname LTb\endcsname%%
      \put(788,9729){\makebox(0,0)[l]{\strut{}\tiny{EITEST-KS}}}%
      \csname LTb\endcsname%%
      \put(788,9609){\makebox(0,0)[l]{\strut{}\tiny{EITEST-MMD}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(2604,9475){\makebox(0,0)[r]{\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(2604,9819){\makebox(0,0)[r]{\strut{}\tiny{0.2}}}%
      \csname LTb\endcsname%%
      \put(2604,10163){\makebox(0,0)[r]{\strut{}\tiny{0.4}}}%
      \csname LTb\endcsname%%
      \put(2604,10507){\makebox(0,0)[r]{\strut{}\tiny{0.6}}}%
      \csname LTb\endcsname%%
      \put(2604,10851){\makebox(0,0)[r]{\strut{}\tiny{0.8}}}%
      \csname LTb\endcsname%%
      \put(2604,11195){\makebox(0,0)[r]{\strut{}\tiny{1}}}%
      \csname LTb\endcsname%%
      \put(2706,9289){\makebox(0,0){\strut{}\tiny{0.01}}}%
      \csname LTb\endcsname%%
      \put(3094,9289){\makebox(0,0){\strut{}\tiny{0.1}}}%
      \csname LTb\endcsname%%
      \put(3482,9289){\makebox(0,0){\strut{}\tiny{1}}}%
      \csname LTb\endcsname%%
      \put(3870,9289){\makebox(0,0){\strut{}\tiny{10}}}%
      \csname LTb\endcsname%%
      \put(4258,9289){\makebox(0,0){\strut{}\tiny{100}}}%
      \csname LTb\endcsname%%
      \put(4646,9289){\makebox(0,0){\strut{}\tiny{1000}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(3676,9010){\makebox(0,0){\strut{}\small{signal-to-noise ratio $r_\text{m}$}}}%
      \csname LTb\endcsname%%
      \put(3676,11560){\makebox(0,0){\strut{}\small{Mean impact model}}}%
      \csname LTb\endcsname%%
      \put(3626,9969){\makebox(0,0)[l]{\strut{}\tiny{GC-VAR}}}%
      \csname LTb\endcsname%%
      \put(3626,9849){\makebox(0,0)[l]{\strut{}\tiny{TE-KSG}}}%
      \csname LTb\endcsname%%
      \put(3626,9729){\makebox(0,0)[l]{\strut{}\tiny{EITEST-KS}}}%
      \csname LTb\endcsname%%
      \put(3626,9609){\makebox(0,0)[l]{\strut{}\tiny{EITEST-MMD}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(204,6515){\makebox(0,0)[r]{\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(204,6859){\makebox(0,0)[r]{\strut{}\tiny{0.2}}}%
      \csname LTb\endcsname%%
      \put(204,7203){\makebox(0,0)[r]{\strut{}\tiny{0.4}}}%
      \csname LTb\endcsname%%
      \put(204,7547){\makebox(0,0)[r]{\strut{}\tiny{0.6}}}%
      \csname LTb\endcsname%%
      \put(204,7891){\makebox(0,0)[r]{\strut{}\tiny{0.8}}}%
      \csname LTb\endcsname%%
      \put(204,8235){\makebox(0,0)[r]{\strut{}\tiny{1}}}%
      \csname LTb\endcsname%%
      \put(306,6329){\makebox(0,0){\strut{}\tiny{1}}}%
      \csname LTb\endcsname%%
      \put(791,6329){\makebox(0,0){\strut{}\tiny{2}}}%
      \csname LTb\endcsname%%
      \put(1276,6329){\makebox(0,0){\strut{}\tiny{4}}}%
      \csname LTb\endcsname%%
      \put(1761,6329){\makebox(0,0){\strut{}\tiny{8}}}%
      \csname LTb\endcsname%%
      \put(2246,6329){\makebox(0,0){\strut{}\tiny{16}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1276,6050){\makebox(0,0){\strut{}\small{variance increase $r_\text{v}$}}}%
      \csname LTb\endcsname%%
      \put(1276,8600){\makebox(0,0){\strut{}\small{Variance impact model}}}%
      \csname LTb\endcsname%%
      \put(1226,7009){\makebox(0,0)[l]{\strut{}\tiny{GC-VAR}}}%
      \csname LTb\endcsname%%
      \put(1226,6889){\makebox(0,0)[l]{\strut{}\tiny{TE-KSG}}}%
      \csname LTb\endcsname%%
      \put(1226,6769){\makebox(0,0)[l]{\strut{}\tiny{EITEST-KS}}}%
      \csname LTb\endcsname%%
      \put(1226,6649){\makebox(0,0)[l]{\strut{}\tiny{EITEST-MMD}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(2604,6515){\makebox(0,0)[r]{\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(2604,6859){\makebox(0,0)[r]{\strut{}\tiny{0.2}}}%
      \csname LTb\endcsname%%
      \put(2604,7203){\makebox(0,0)[r]{\strut{}\tiny{0.4}}}%
      \csname LTb\endcsname%%
      \put(2604,7547){\makebox(0,0)[r]{\strut{}\tiny{0.6}}}%
      \csname LTb\endcsname%%
      \put(2604,7891){\makebox(0,0)[r]{\strut{}\tiny{0.8}}}%
      \csname LTb\endcsname%%
      \put(2604,8235){\makebox(0,0)[r]{\strut{}\tiny{1}}}%
      \csname LTb\endcsname%%
      \put(2753,6329){\makebox(0,0){\strut{}\tiny{3}}}%
      \csname LTb\endcsname%%
      \put(3226,6329){\makebox(0,0){\strut{}\tiny{4}}}%
      \csname LTb\endcsname%%
      \put(3700,6329){\makebox(0,0){\strut{}\tiny{5}}}%
      \csname LTb\endcsname%%
      \put(4173,6329){\makebox(0,0){\strut{}\tiny{6}}}%
      \csname LTb\endcsname%%
      \put(4646,6329){\makebox(0,0){\strut{}\tiny{7}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(3676,6050){\makebox(0,0){\strut{}\small{degrees of freedom $r_\text{t}$}}}%
      \csname LTb\endcsname%%
      \put(3676,8600){\makebox(0,0){\strut{}\small{Tail impact model}}}%
      \csname LTb\endcsname%%
      \put(3626,8187){\makebox(0,0)[l]{\strut{}\tiny{GC-VAR}}}%
      \csname LTb\endcsname%%
      \put(3626,8067){\makebox(0,0)[l]{\strut{}\tiny{TE-KSG}}}%
      \csname LTb\endcsname%%
      \put(3626,7947){\makebox(0,0)[l]{\strut{}\tiny{EITEST-KS}}}%
      \csname LTb\endcsname%%
      \put(3626,7827){\makebox(0,0)[l]{\strut{}\tiny{EITEST-MMD}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(204,3555){\makebox(0,0)[r]{\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(204,3899){\makebox(0,0)[r]{\strut{}\tiny{0.2}}}%
      \csname LTb\endcsname%%
      \put(204,4243){\makebox(0,0)[r]{\strut{}\tiny{0.4}}}%
      \csname LTb\endcsname%%
      \put(204,4588){\makebox(0,0)[r]{\strut{}\tiny{0.6}}}%
      \csname LTb\endcsname%%
      \put(204,4932){\makebox(0,0)[r]{\strut{}\tiny{0.8}}}%
      \csname LTb\endcsname%%
      \put(204,5276){\makebox(0,0)[r]{\strut{}\tiny{1}}}%
      \csname LTb\endcsname%%
      \put(306,3369){\makebox(0,0){\strut{}\tiny{8}}}%
      \csname LTb\endcsname%%
      \put(583,3369){\makebox(0,0){\strut{}\tiny{16}}}%
      \csname LTb\endcsname%%
      \put(860,3369){\makebox(0,0){\strut{}\tiny{32}}}%
      \csname LTb\endcsname%%
      \put(1137,3369){\makebox(0,0){\strut{}\tiny{64}}}%
      \csname LTb\endcsname%%
      \put(1415,3369){\makebox(0,0){\strut{}\tiny{128}}}%
      \csname LTb\endcsname%%
      \put(1692,3369){\makebox(0,0){\strut{}\tiny{256}}}%
      \csname LTb\endcsname%%
      \put(1969,3369){\makebox(0,0){\strut{}\tiny{512}}}%
      \csname LTb\endcsname%%
      \put(2246,3369){\makebox(0,0){\strut{}\tiny{1024}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1276,3090){\makebox(0,0){\strut{}\small{number of events $N$}}}%
      \csname LTb\endcsname%%
      \put(1276,5641){\makebox(0,0){\strut{}\small{Variance impact model}}}%
      \csname LTb\endcsname%%
      \put(1226,4049){\makebox(0,0)[l]{\strut{}\tiny{GC-VAR}}}%
      \csname LTb\endcsname%%
      \put(1226,3929){\makebox(0,0)[l]{\strut{}\tiny{TE-KSG}}}%
      \csname LTb\endcsname%%
      \put(1226,3809){\makebox(0,0)[l]{\strut{}\tiny{EITEST-KS}}}%
      \csname LTb\endcsname%%
      \put(1226,3689){\makebox(0,0)[l]{\strut{}\tiny{EITEST-MMD}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(2604,3555){\makebox(0,0)[r]{\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(2604,3899){\makebox(0,0)[r]{\strut{}\tiny{0.2}}}%
      \csname LTb\endcsname%%
      \put(2604,4243){\makebox(0,0)[r]{\strut{}\tiny{0.4}}}%
      \csname LTb\endcsname%%
      \put(2604,4588){\makebox(0,0)[r]{\strut{}\tiny{0.6}}}%
      \csname LTb\endcsname%%
      \put(2604,4932){\makebox(0,0)[r]{\strut{}\tiny{0.8}}}%
      \csname LTb\endcsname%%
      \put(2604,5276){\makebox(0,0)[r]{\strut{}\tiny{1}}}%
      \csname LTb\endcsname%%
      \put(2706,3369){\makebox(0,0){\strut{}\tiny{8}}}%
      \csname LTb\endcsname%%
      \put(2979,3369){\makebox(0,0){\strut{}\tiny{16}}}%
      \csname LTb\endcsname%%
      \put(3252,3369){\makebox(0,0){\strut{}\tiny{32}}}%
      \csname LTb\endcsname%%
      \put(3525,3369){\makebox(0,0){\strut{}\tiny{64}}}%
      \csname LTb\endcsname%%
      \put(3798,3369){\makebox(0,0){\strut{}\tiny{128}}}%
      \csname LTb\endcsname%%
      \put(4072,3369){\makebox(0,0){\strut{}\tiny{256}}}%
      \csname LTb\endcsname%%
      \put(4345,3369){\makebox(0,0){\strut{}\tiny{512}}}%
      \csname LTb\endcsname%%
      \put(4618,3369){\makebox(0,0){\strut{}\tiny{1024}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(3676,3090){\makebox(0,0){\strut{}\small{number of events $N$}}}%
      \csname LTb\endcsname%%
      \put(3676,5641){\makebox(0,0){\strut{}\small{Tail impact model}}}%
      \csname LTb\endcsname%%
      \put(3188,5228){\makebox(0,0)[l]{\strut{}\tiny{GC-VAR}}}%
      \csname LTb\endcsname%%
      \put(3188,5108){\makebox(0,0)[l]{\strut{}\tiny{TE-KSG}}}%
      \csname LTb\endcsname%%
      \put(3188,4988){\makebox(0,0)[l]{\strut{}\tiny{EITEST-KS}}}%
      \csname LTb\endcsname%%
      \put(3188,4868){\makebox(0,0)[l]{\strut{}\tiny{EITEST-MMD}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(204,595){\makebox(0,0)[r]{\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(204,939){\makebox(0,0)[r]{\strut{}\tiny{0.2}}}%
      \csname LTb\endcsname%%
      \put(204,1283){\makebox(0,0)[r]{\strut{}\tiny{0.4}}}%
      \csname LTb\endcsname%%
      \put(204,1628){\makebox(0,0)[r]{\strut{}\tiny{0.6}}}%
      \csname LTb\endcsname%%
      \put(204,1972){\makebox(0,0)[r]{\strut{}\tiny{0.8}}}%
      \csname LTb\endcsname%%
      \put(204,2316){\makebox(0,0)[r]{\strut{}\tiny{1}}}%
      \csname LTb\endcsname%%
      \put(306,409){\makebox(0,0){\strut{}\tiny{1024}}}%
      \csname LTb\endcsname%%
      \put(941,409){\makebox(0,0){\strut{}\tiny{2048}}}%
      \csname LTb\endcsname%%
      \put(1577,409){\makebox(0,0){\strut{}\tiny{4096}}}%
      \csname LTb\endcsname%%
      \put(2212,409){\makebox(0,0){\strut{}\tiny{8192}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1276,130){\makebox(0,0){\strut{}\small{time series length $T$}}}%
      \csname LTb\endcsname%%
      \put(1276,2681){\makebox(0,0){\strut{}\small{Variance impact model}}}%
      \csname LTb\endcsname%%
      \put(1226,1089){\makebox(0,0)[l]{\strut{}\tiny{GC-VAR}}}%
      \csname LTb\endcsname%%
      \put(1226,969){\makebox(0,0)[l]{\strut{}\tiny{TE-KSG}}}%
      \csname LTb\endcsname%%
      \put(1226,849){\makebox(0,0)[l]{\strut{}\tiny{EITEST-KS}}}%
      \csname LTb\endcsname%%
      \put(1226,729){\makebox(0,0)[l]{\strut{}\tiny{EITEST-MMD}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(2604,595){\makebox(0,0)[r]{\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(2604,939){\makebox(0,0)[r]{\strut{}\tiny{0.2}}}%
      \csname LTb\endcsname%%
      \put(2604,1283){\makebox(0,0)[r]{\strut{}\tiny{0.4}}}%
      \csname LTb\endcsname%%
      \put(2604,1628){\makebox(0,0)[r]{\strut{}\tiny{0.6}}}%
      \csname LTb\endcsname%%
      \put(2604,1972){\makebox(0,0)[r]{\strut{}\tiny{0.8}}}%
      \csname LTb\endcsname%%
      \put(2604,2316){\makebox(0,0)[r]{\strut{}\tiny{1}}}%
      \csname LTb\endcsname%%
      \put(2706,409){\makebox(0,0){\strut{}\tiny{2048}}}%
      \csname LTb\endcsname%%
      \put(3353,409){\makebox(0,0){\strut{}\tiny{4096}}}%
      \csname LTb\endcsname%%
      \put(3999,409){\makebox(0,0){\strut{}\tiny{8192}}}%
      \csname LTb\endcsname%%
      \put(4646,409){\makebox(0,0){\strut{}\tiny{16384}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(3676,130){\makebox(0,0){\strut{}\small{time series length $T$}}}%
      \csname LTb\endcsname%%
      \put(3676,2681){\makebox(0,0){\strut{}\small{Tail impact model}}}%
      \csname LTb\endcsname%%
      \put(3626,1089){\makebox(0,0)[l]{\strut{}\tiny{GC-VAR}}}%
      \csname LTb\endcsname%%
      \put(3626,969){\makebox(0,0)[l]{\strut{}\tiny{TE-KSG}}}%
      \csname LTb\endcsname%%
      \put(3626,849){\makebox(0,0)[l]{\strut{}\tiny{EITEST-KS}}}%
      \csname LTb\endcsname%%
      \put(3626,729){\makebox(0,0)[l]{\strut{}\tiny{EITEST-MMD}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{ms-gnuplottex-fig2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> ms-gnuplottex-fig3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4800.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(663,1886){\makebox(0,0)[r]{\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(663,2047){\makebox(0,0)[r]{\strut{}\tiny{200}}}%
      \csname LTb\endcsname%%
      \put(663,2209){\makebox(0,0)[r]{\strut{}\tiny{400}}}%
      \csname LTb\endcsname%%
      \put(663,2370){\makebox(0,0)[r]{\strut{}\tiny{600}}}%
      \csname LTb\endcsname%%
      \put(663,2532){\makebox(0,0)[r]{\strut{}\tiny{800}}}%
      \csname LTb\endcsname%%
      \put(663,2693){\makebox(0,0)[r]{\strut{}\tiny{1000}}}%
      \csname LTb\endcsname%%
      \put(1019,1626){\makebox(0,0){\strut{}\tiny{12h}}}%
      \csname LTb\endcsname%%
      \put(1338,1626){\makebox(0,0){\strut{}\tiny{18h}}}%
      \csname LTb\endcsname%%
      \put(1657,1626){\makebox(0,0){\strut{}\tiny{00h}}}%
      \csname LTb\endcsname%%
      \put(1976,1626){\makebox(0,0){\strut{}\tiny{06h}}}%
      \csname LTb\endcsname%%
      \put(2295,1626){\makebox(0,0){\strut{}\tiny{12h}}}%
      \csname LTb\endcsname%%
      \put(2614,1626){\makebox(0,0){\strut{}\tiny{18h}}}%
      \csname LTb\endcsname%%
      \put(2933,1626){\makebox(0,0){\strut{}\tiny{00h}}}%
      \csname LTb\endcsname%%
      \put(3252,1626){\makebox(0,0){\strut{}\tiny{06h}}}%
      \csname LTb\endcsname%%
      \put(3571,1626){\makebox(0,0){\strut{}\tiny{12h}}}%
      \csname LTb\endcsname%%
      \put(3890,1626){\makebox(0,0){\strut{}\tiny{18h}}}%
      \csname LTb\endcsname%%
      \put(4209,1626){\makebox(0,0){\strut{}\tiny{00h}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(2759,2526){\makebox(0,0)[l]{\strut{}\scriptsize{clothes washer (CWE)}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(663,446){\makebox(0,0)[r]{\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(663,581){\makebox(0,0)[r]{\strut{}\tiny{1500}}}%
      \csname LTb\endcsname%%
      \put(663,715){\makebox(0,0)[r]{\strut{}\tiny{3000}}}%
      \csname LTb\endcsname%%
      \put(663,850){\makebox(0,0)[r]{\strut{}\tiny{4500}}}%
      \csname LTb\endcsname%%
      \put(663,985){\makebox(0,0)[r]{\strut{}\tiny{6000}}}%
      \csname LTb\endcsname%%
      \put(663,1119){\makebox(0,0)[r]{\strut{}\tiny{7500}}}%
      \csname LTb\endcsname%%
      \put(663,1254){\makebox(0,0)[r]{\strut{}\tiny{9000}}}%
      \csname LTb\endcsname%%
      \put(1019,186){\makebox(0,0){\strut{}\tiny{12h}}}%
      \csname LTb\endcsname%%
      \put(1338,186){\makebox(0,0){\strut{}\tiny{18h}}}%
      \csname LTb\endcsname%%
      \put(1657,186){\makebox(0,0){\strut{}\tiny{00h}}}%
      \csname LTb\endcsname%%
      \put(1976,186){\makebox(0,0){\strut{}\tiny{06h}}}%
      \csname LTb\endcsname%%
      \put(2295,186){\makebox(0,0){\strut{}\tiny{12h}}}%
      \csname LTb\endcsname%%
      \put(2614,186){\makebox(0,0){\strut{}\tiny{18h}}}%
      \csname LTb\endcsname%%
      \put(2933,186){\makebox(0,0){\strut{}\tiny{00h}}}%
      \csname LTb\endcsname%%
      \put(3252,186){\makebox(0,0){\strut{}\tiny{06h}}}%
      \csname LTb\endcsname%%
      \put(3571,186){\makebox(0,0){\strut{}\tiny{12h}}}%
      \csname LTb\endcsname%%
      \put(3890,186){\makebox(0,0){\strut{}\tiny{18h}}}%
      \csname LTb\endcsname%%
      \put(4209,186){\makebox(0,0){\strut{}\tiny{00h}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(2912,1087){\makebox(0,0)[l]{\strut{}\scriptsize{whole house (WHE)}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{ms-gnuplottex-fig3}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> ms-gnuplottex-fig4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4800.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(663,1886){\makebox(0,0)[r]{\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(663,2047){\makebox(0,0)[r]{\strut{}\tiny{500}}}%
      \csname LTb\endcsname%%
      \put(663,2209){\makebox(0,0)[r]{\strut{}\tiny{1000}}}%
      \csname LTb\endcsname%%
      \put(663,2370){\makebox(0,0)[r]{\strut{}\tiny{1500}}}%
      \csname LTb\endcsname%%
      \put(663,2532){\makebox(0,0)[r]{\strut{}\tiny{2000}}}%
      \csname LTb\endcsname%%
      \put(663,2693){\makebox(0,0)[r]{\strut{}\tiny{2500}}}%
      \csname LTb\endcsname%%
      \put(765,1626){\makebox(0,0){\strut{}\tiny{2014-01}}}%
      \csname LTb\endcsname%%
      \put(1691,1626){\makebox(0,0){\strut{}\tiny{2014-07}}}%
      \csname LTb\endcsname%%
      \put(2628,1626){\makebox(0,0){\strut{}\tiny{2015-01}}}%
      \csname LTb\endcsname%%
      \put(3554,1626){\makebox(0,0){\strut{}\tiny{2015-07}}}%
      \csname LTb\endcsname%%
      \put(4490,1626){\makebox(0,0){\strut{}\tiny{2016-01}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(2555,2526){\makebox(0,0)[l]{\strut{}\scriptsize{all earthquakes (globally)}}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(663,446){\makebox(0,0)[r]{\strut{}\tiny{0}}}%
      \csname LTb\endcsname%%
      \put(663,608){\makebox(0,0)[r]{\strut{}\tiny{500}}}%
      \csname LTb\endcsname%%
      \put(663,769){\makebox(0,0)[r]{\strut{}\tiny{1000}}}%
      \csname LTb\endcsname%%
      \put(663,931){\makebox(0,0)[r]{\strut{}\tiny{1500}}}%
      \csname LTb\endcsname%%
      \put(663,1092){\makebox(0,0)[r]{\strut{}\tiny{2000}}}%
      \csname LTb\endcsname%%
      \put(663,1254){\makebox(0,0)[r]{\strut{}\tiny{2500}}}%
      \csname LTb\endcsname%%
      \put(765,186){\makebox(0,0){\strut{}\tiny{2014-01}}}%
      \csname LTb\endcsname%%
      \put(1691,186){\makebox(0,0){\strut{}\tiny{2014-07}}}%
      \csname LTb\endcsname%%
      \put(2628,186){\makebox(0,0){\strut{}\tiny{2015-01}}}%
      \csname LTb\endcsname%%
      \put(3554,186){\makebox(0,0){\strut{}\tiny{2015-07}}}%
      \csname LTb\endcsname%%
      \put(4490,186){\makebox(0,0){\strut{}\tiny{2016-01}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(2861,1087){\makebox(0,0)[l]{\strut{}\scriptsize{earthquakes in China}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{ms-gnuplottex-fig4}}%
    \gplfronttext
  \end{picture}%
\endgroup

